Improving Distantly Supervised Relation Extraction by Natural Language Inference

To reduce human annotations for relation extraction (RE) tasks, distantly supervised approaches have been proposed, while struggling with low performance. In this work, we propose a novel DSRE-NLI framework, which considers both distant supervision from existing knowledge bases and indirect supervision from pretrained language models for other tasks. DSRE-NLI energizes an off-the-shelf natural language inference (NLI) engine with a semi-automatic relation verbalization (SARV) mechanism to provide indirect supervision and further consolidates the distant annotations to benefit multi-classification RE models. The NLI-based indirect supervision acquires only one relation verbalization template from humans as a semantically general template for each relationship, and then the template set is enriched by high-quality textual patterns automatically mined from the distantly annotated corpus. With two simple and effective data consolidation strategies, the quality of training data is substantially improved. Extensive experiments demonstrate that the proposed framework significantly improves the SOTA performance (up to 7.73\% of F1) on distantly supervised RE benchmark datasets.

==> outline.tex <==
\section{outline}

Title (not sure): 

    1. Sentence-level relation extraction with distant and indirect supervision signals
    2. Distant and indirect supervision for sentence-level relation extraction
    3. Weakly supervised sentence-level relation extraction via distant and indirect signals
    (or any other perspectives)

Introduction:
    
    1. Sentence-level RE task 
        i. definition and why it's important in information extraction tasks (references: first paragraph of \citep{zheng2019diag}, \cite{jia2019arnor}, \cite{ma2021sent})
        
    2. Three lines: supervised methods, distantly supervised methods (e.g., sentence level denoise, and bag level denoise), Indirectly supervised methods
        i. supervised methods (references: \cite{zhang2017position}, \cite{zeng2014relation},  \cite{dos2015classifying}, \cite{zhou2016attention}, \cite{zelenko2003kernel}, \cite{joshi2020spanbert}, \cite{yamada2020luke}, \cite{zhang2019ernie}, \cite{peters2019knowledge}, \cite{wang2021k}, \cite{soares2019matching}, \cite{zhou2021improved}, \cite{chen2022knowprompt})
        ii. distantly supervised methods (assumption: If two entities participate in a relation, all sentences that mention these two entities express that relation. labeling errors: FP and FN, draw a figure with examples)
            a. bag-level settings with various denoising strategies (Expressed-at-least-once assumption: If two entities participate in a relation, at least one sentence that mentions these two entities might express that relation.) (references: \cite{mintz2009distant}, \cite{riedel2010modeling}, \cite{hoffmann2011knowledge}, \cite{surdeanu2012multi}, \cite{zeng2015distant}, \cite{lin2016neural}, \cite{jiang2018revisiting}, \cite{qin2018robust}, \cite{he2020improving})
            b. sentence-level setting with various denoising strategies (mention the reason why back to the sentence-level setting which is adopted by supervised methods: "bag-level suffers from two limitations: 1) Unable to handle the sentence-level prediction; 2) Sensitive to the bags with all noisy sentences which do not describe a relation at all."-- quoted from \cite{feng2018reinforcement}) (other references: \citep{zheng2019diag}, \cite{jia2019arnor}, \cite{ma2021sent}) 
        iii. indirectly supervised methods (mainly taking advantage of pre-trained language models)
            a. \cite{obamuyide2018zero} is the first work relating relation classification to textual entailment, but "but only evaluate performance as binary entailment, not as a RE task" -- quoted from \cite{sainz2021label}, in zero-shot
            b. \cite{sainz2021label} formally reformulates RE into textual entailment task, in zero- and few-shot
            c. \cite{lu2022summarization} formally reformulates RE into text summarization task, in zero- and few-shot
            
    3. Our motivations: 
        i. supervised methods require huge of human efforts for annotating 
        ii. distantly supervised methods are struggling with noisy labels, SOTA performance still falls a lot behind that in supervised settings.
        iii. issues with indirectly supervised methods: 
            a. zero-shot suffers low performance
            b. although few-shot with 1\% human labeled training data requires much less human efforts than that in supervised settings to annotate, it still needs around 16 (TACRED) or 370 (NYT) manually labeled samples for each relation, and suffers low performance. If few-shot intends to achieve satisfactory performance, it needs around 10\% human labeled training data to be used in fine-tuning, which means around 160 (TACRED) or 3700 (NYT) labeled samples. Therefore, indirectly supervised methods with acceptable performance still require a lot of human efforts.
        
        We propose a novel weakly supervised setting for sentence-level RE where only a little human efforts can bring good performance by jointly taking advantage of distant supervision and indirect supervision. 
            a. pattern mining from distant labels given by KBs
            b. seeding + pattern grouping to provide high quality relation label verbalization templates for MNLI (fine-tuning MNLI is not appropriate in weakly supervised settings)
            c. Jointly using distant labels and MNLI predictions to train traditional multi-classification RE models.

  
Related work:

    1. distant supervision methods
        i. bag-level (\cite{mintz2009distant}, \cite{riedel2010modeling}, \cite{hoffmann2011knowledge}, \cite{surdeanu2012multi}, \cite{zeng2015distant}, \cite{lin2016neural}, \cite{qin2018robust}, \cite{he2020improving})
        ii. sentence-level (\cite{feng2018reinforcement}, \citep{zheng2019diag}, \cite{jia2019arnor}, \cite{ma2021sent})
        iii. our method belongs to sentence-level
    2. Indirect supervision methods
        i. \cite{levy2017zero} RE --> QA, in zero-shot 
        ii. \cite{obamuyide2018zero}, \cite{sainz2021label} RE --> textual entailment, in zero- and few-shot
        iii. \cite{lu2022summarization} RE --> text summarization, in zero- and few-shot
        iv. we use textual entailment because: 
            a. label verbalization templates can be directly obtained from pattern mining on distantly labeled corpus, while question templates in RE --> QA can not.
            b. Inference step from textual entailment to RE is easier than that from text summarization to RE
    
Method:
    
    1. Pattern mining and pattern grouping (examples, algorithm, definition of semantic duplication and underlying assumptions)
    2. MC models using newly generate training data
    
Experiments:

    1. datasets (NYTs, simulated TACRED)
    2. baselines
    3. results:
        i. fine-tuning MNLI is not working well in weakly supervised settings
        ii. statistics for pattern mining and pattern grouping
        iii. one seed + patterns for MNLI
        iv. mc on newly generated training data
        v. ablation study:
            a. one seed
            b. one pattern (or multiple patterns)
            
--------------------------------------------------------------------------------------------------------
            
    
Problem:

    sentence-level RE in weakly supervised settings
        1). discuss sentence-level RE is important
        2). discuss distant supervision settings (including denoise strategies)
        3). discuss indirect supervision settings (cast the target task into a formulation which allows to exploit the knowledge implicit in pre-trained LM (prompt-based) or general-purpose question answering or entailment engines (pivot tasks))

Related work:

    DS-RE methods and MNLI for few-shot RE
    
Motivations:

    1. There is no need much human efforts in weakly supervised settings, which is desired in real world applications. However, SOTA RE performance in weakly supervised settings is still significantly worse than that in fully supervised settings. We observed that supervision sources (signals) have not been fully explored, mainly rely on knowledge bases (hard labeling). We attempt to utilize both distant and indirect supervisions. 
    
Methodology:

    1. Supervision sources: knowledge bases and pre-trained language models for textual entailment
    2. For KB labeling, we follow the traditional assumption.
    3. For reformulating RE as textual entailment, unlike in supervised settings, there is no data with ground-truth labels for model fine-tuning in weakly supervised settings, which makes generating high quality (no redundancy and specific to the target domain) label verbalization templates more essential than ever before. 
        1). Drawbacks with human experts writing label verbalization templates:
            a. time consuming
            b. prone to be redundant (semantically duplicated), using examples
            c. prone to be general (lack of diversity), using examples
        2). Propose a semi-automatic approach to generate high quality label verbalization templates by pattern mining and pattern grouping
            a. seed
            b. pattern mining and pattern grouping provide high quality pattern candidates
    4. Pre-trained language models for textual entailment with semi-automatically generated label verbalization templates can be used as a labeling source for training data. We jointly take advantage of the two labeling sources, which can provide higher quality training data for traditional MC models to capture particular semantic features with entity position information for each pre-defined relation. 
    
% Experiments:

%     1. One template for TACRED and fine-tune MNLI with training data. If the zero-shot result is much worse than that of using multiple templates, and the fine-tuning result is close to using multiple templates, then we can say that the number of templates is not the key in supervised settings, but fine-tuning with training data with high quality labels is. However, in weakly supervised settings, there is no training data with high quality labels for fine-tuning. The diversity of templates for each relation will be the bottleneck in these settings, which has a significant impact on the textual entailment prediction.
%     2. the highest frequent pattern from initial patterns (and topk patterns) --> one seed --> one seed + selected patterns (after pattern grouping)
%     3. training MC models with newly generated training data


